The Onset of Thermally Unstable Cooling from the Hot Atmospheres of Giant Galaxies in Clusters - Constraints on Feedback Models

We present accurate mass and thermodynamic profiles for a sample of 56 galaxy clusters observed with the Chandra X-ray Observatory. We investigate the effects of local gravitational acceleration in central cluster galaxies, and we explore the role of the local free-fall time (t$_{\rm ff}$) in thermally unstable cooling. We find that the local cooling time (t$_{\rm cool}$) is as effective an indicator of cold gas, traced through its nebular emission, as the ratio of t$_{\rm cool}$/t$_{\rm ff}$. Therefore, t$_{\rm cool}$ alone apparently governs the onset of thermally unstable cooling in hot atmospheres. The location of the minimum t$_{\rm cool}$/t$_{\rm ff}$, a thermodynamic parameter that simulations suggest may be key in driving thermal instability, is unresolved in most systems. As a consequence, selection effects bias the value and reduce the observed range in measured t$_{\rm cool}$/t$_{\rm ff}$ minima. The entropy profiles of cool-core clusters are characterized by broken power-laws down to our resolution limit, with no indication of isentropic cores. We show, for the first time, that mass isothermality and the $K \propto r^{2/3}$ entropy profile slope imply a floor in t$_{\rm cool}$/t$_{\rm ff}$ profiles within central galaxies. No significant departures of t$_{\rm cool}$/t$_{\rm ff}$ below 10 are found, which is inconsistent with many recent feedback models. The inner densities and cooling times of cluster atmospheres are resilient to change in response to powerful AGN activity, suggesting that the energy coupling between AGN heating and atmospheric gas is gentler than most models predict.

==> defn.tex <==
%-*-LaTeX-*-
% Copied from gmorris
% Note that some of these call others, eg \kmps uses \km.

% journals
%\newcommand{\apj}{ApJ}
%\newcommand{\mnras}{MNRAS}
%\newcommand{\nat}{Nat}
%\newcommand{\physrevB}{Phys. Rev. B}
%\newcommand{\araa}{ARA\&A}                % "Ann. Rev. Astron. Astrophys."
%\newcommand{\aap}{A\&A}                   % "Astron. Astrophys."
%\newcommand{\aaps}{A\&AS}                 % "Astron. Astrophys. Suppl. Ser."
%\newcommand{\aj}{AJ}                      % "Astron. J."
%\newcommand{\apjs}{ApJS}                  % "Astrophys. J. Suppl. Ser."
%\newcommand{\pasp}{PASP}                  % "Publ. Astron. Soc. Pac."
%\newcommand{\apjl}{ApJ}                   % letter at ApJ
%\newcommand{\pasj}{PASJ}
%\newcommand{\gca}{Geochim. Cosmochim. Acta}
%\newcommand{\physrep}{Phys. Rep.}
%\newcommand{\aapr}{A\&A Rev.}
%\newcommand{\ssr}{Space Sci. Rev.}
%\newcommand{\na}{New Astron.}
%\newcommand{\nar}{NewA Rev.}
%\newcommand{\jgr}{J. Geophys. Res.}

% Length
\newcommand{\Mpc}{\rm\; Mpc}
\newcommand{\kpc}{\rm\; kpc}
\newcommand{\pc}{\rm\; pc}
\newcommand{\km}{\rm\; km}
\newcommand{\m}{\rm\; m}
\newcommand{\cm}{\rm\; cm}
\newcommand{\mum}{\hbox{$\rm\; \mu m\,$}}
\newcommand{\pix}{\rm\; pixel}
%
\newcommand{\cmps}{\hbox{$\cm\s^{-1}\,$}}
\newcommand{\cmpssq}{\hbox{$\cm\s^{-2}\,$}}
\newcommand{\cmsq}{\hbox{$\cm^2\,$}}
\newcommand{\cmcu}{\hbox{$\cm^3\,$}}
\newcommand{\pcmcuK}{\hbox{$\cm^{-3}\K\,$}}
\newcommand{\ppix}{\hbox{$\pix^{-1}\,$}}
\newcommand{\ppixsq}{\hbox{$\pix^{-2}\,$}}
\newcommand{\kpcsq}{\hbox{$\kpc^{2}\,$}}
% Length


% Time
\newcommand{\hr}{\rm\; hr}
\newcommand{\yr}{\rm\; yr}
\newcommand{\Gyr}{\rm\; Gyr}
\newcommand{\Myr}{\rm\; Myr}
\newcommand{\s}{\rm\; s}
\newcommand{\ms}{\rm\; ms}
\newcommand{\ks}{\rm\; ks}
\newcommand{\mus}{\hbox{$\rm\; \mu s\,$}}
% Time


% Frequency
\newcommand{\GHz}{\rm\; GHz}
\newcommand{\MHz}{\rm\; MHz}
\newcommand{\Hz}{\rm\; Hz}
% Frequency


% Temperature
\newcommand{\K}{\rm\; K}
% Temperature


% Pressure
\newcommand{\Kpcmc}{\hbox{$\K\cm^{-3}\,$}}
\newcommand{\keVpcmcu}{\hbox{$\keV\cm^{-3}\,$}}
% Pressure


% Mass
\newcommand{\g}{\rm\; g}
%
\newcommand{\gpcm}{\hbox{$\g\cm^{-3}\,$}}
\newcommand{\gpcmps}{\hbox{$\g\cm^{-3}\s^{-1}\,$}}
\newcommand{\gps}{\hbox{$\g\s^{-1}\,$}}
%
\newcommand{\Msun}{\hbox{$\rm\thinspace M_{\odot}$}}
\newcommand{\Msunpc}{\hbox{$\Msun\pc^{-3}\,$}}
\newcommand{\Msunpkpc}{\hbox{$\Msun\kpc^{-1}\,$}}
\newcommand{\Msunppc}{\hbox{$\Msun\pc^{-3}\,$}}
\newcommand{\Msunppcpyr}{\hbox{$\Msun\pc^{-3}\yr^{-1}\,$}}
\newcommand{\Msunpyr}{\hbox{$\Msun\yr^{-1}\,$}}
% Mass


% Energy
\newcommand{\MeV}{\rm\; MeV}
\newcommand{\keV}{\rm\; keV}
\newcommand{\eV}{\rm\; eV}
\newcommand{\erg}{\rm\; erg}
\newcommand{\Jy}{\rm\; Jy}
\newcommand{\mJy}{\rm\; mJy}
\newcommand{\W}{\rm\; W}
%
\newcommand{\ergcmcups}{\hbox{$\erg\cm^3\ps\,$}}
\newcommand{\ergpcmps}{\hbox{$\erg\cm^{-3}\s^{-1}\,$}}
\newcommand{\ergpcmsq}{\hbox{$\erg\cm^{-2}\,$}}
\newcommand{\ergpcmcu}{\hbox{$\erg\cm^{-3}\,$}}
\newcommand{\ergpcmsqps}{\hbox{$\erg\cm^{-2}\s^{-1}\,$}}
\newcommand{\ergpcmsqpspA}{\hbox{$\erg\cm^{-2}\s^{-1}$\AA$^{-1}\,$}}
\newcommand{\ergpcmsqpspsr}{\hbox{$\erg\cm^{-2}\s^{-1}\sr^{-1}\,$}}
\newcommand{\ergpcmcups}{\hbox{$\erg\cm^{-3}\s^{-1}\,$}}
\newcommand{\ergps}{\hbox{$\erg\s^{-1}\,$}}
\newcommand{\ergpspHz}{\hbox{$\erg\s^{-1}\pHz\,$}}
\newcommand{\ergpspmp}{\hbox{$\erg\s^{-1}\Mpc^{-3}\,$}}
\newcommand{\ergpspkpc}{\hbox{$\erg\s^{-1}\kpc^{-1}\,$}}
%
\newcommand{\keVpcmsqpspsr}{\hbox{$\keV\cm^{-2}\s^{-1}\sr^{-1}\,$}}
%
\newcommand{\WpHzpsr}{\hbox{$\W\pHz\psr\,$}}
\newcommand{\WpHz}{\hbox{$\W\pHz\,$}}
%
\newcommand{\surbri}{\hbox{$\rm\thinspace photons\pcmsq\ps\pasecsq$}}
\newcommand{\expmapcorr}{\hbox{$\rm\thinspace photons\pcmsq\ps\ppix$}}
% Energy


% Force
\newcommand{\dyn}{\rm\; dyn}
\newcommand{\dynpcmsq}{\hbox{$\dyn\cm^{-2}\,$}}
% Force


% Speed
\newcommand{\kmps}{\hbox{$\km\s^{-1}\,$}}
\newcommand{\kmpspmp}{\hbox{$\km\s^{-1}\Mpc{-1}\,$}}
\newcommand{\kmpspMpc}{\hbox{$\kmps\Mpc^{-1}\,$}}
% Speed


% Luminosity
\newcommand{\Lsun}{\hbox{$\rm\thinspace L_{\odot}$}}
\newcommand{\Lsunppc}{\hbox{$\Lsun\pc^{-3}\,$}}
% Luminosity


% Misc
\newcommand{\dex}{\rm\; dex}

\newcommand{\plawnorm}{\hbox{$\rm\thinspace photons\keV^{-1}\cm^{-2}\s^{-1}\,$}}
\newcommand{\Zsun}{\hbox{$\thinspace \mathrm{Z}_{\odot}$}}

\newcommand{\gauss}{\rm\; gauss}
\newcommand{\muG}{\hbox{$\rm\thinspace {\mu}\mathrm{G}$}}
%
\newcommand{\chisq}{\hbox{$\chi^2$}}
\newcommand{\delchi}{\hbox{$\Delta\chi$}}
%
\newcommand{\ph}{\rm\; ph}
% Misc

% Angles
\newcommand{\amin}{\rm\; arcmin}
\newcommand{\aminsq}{\hbox{$\amin^{2}\,$}}
\newcommand{\asec}{\rm\; arcsec}
\newcommand{\asecsq}{\hbox{$\asec^{2}\,$}}
\newcommand{\sr}{\rm\; sr}
\newcommand{\degword}{\rm\; deg}
\newcommand{\degsq}{\hbox{$\degword^2\,$}}
% Angles

% Emission measure
\newcommand{\emm}{\hbox{$\cm^{-5}\,$}}
\newcommand{\sqremm}{\hbox{$\cm^{-5/2}\,$}}
\newcommand{\empasecsq}{\hbox{$\emm\asec^{-2}\,$}}
\newcommand{\keVempasecsq}{\hbox{$\keV\emm\asec^{-2}\,$}}
\newcommand{\pseudoP}{\hbox{$\keV\sqremm\asec^{-2}\,$}}
% Emission measure

% Per something
\newcommand{\pcm}{\hbox{$\cm^{-1}\,$}}
\newcommand{\psqcm}{\hbox{$\cm^{-2}\,$}}
\newcommand{\pcmsq}{\hbox{$\cm^{-2}\,$}}
\newcommand{\pcmcu}{\hbox{$\cm^{-3}\,$}}
\newcommand{\pcmcus}{\hbox{$\pcmcu\s\,$}}
\newcommand{\pmpc}{\hbox{$\Mpc^{-1}\,$}}
\newcommand{\pmpccu}{\hbox{$\Mpc^{-3}\,$}}
\newcommand{\ps}{\hbox{$\s^{-1}\,$}}
\newcommand{\pHz}{\hbox{$\Hz^{-1}\,$}}
\newcommand{\pcmK}{\hbox{$\cm^{-3}\K$}}
\newcommand{\phpcmsqps}{\hbox{$\ph\cm^{-2}\s^{-1}\,$}}
\newcommand{\psr}{\hbox{$\sr^{-1}\,$}}
\newcommand{\pasecsq}{\hbox{$\asec^{-2}\,$}}
% Per something

% Use times for maths fonts
% \DeclareSymbolFont{operators}   {OT1}{ptmcm}{m}{n}
% \DeclareSymbolFont{letters}     {OML}{ptmcm}{m}{it}
% \SetMathAlphabet{\mathbf}{normal}{\encodingdefault}{\rmdefault}{\bfdefault}{n}%
% \SetMathAlphabet{\mathsf}{normal}{\encodingdefault}{\sfdefault}{m}{n}%
% \SetMathAlphabet{\mathrm}{normal}{\encodingdefault}{\rmdefault}{m}{n}%
% \SetSymbolFont{operators}{bold}{OT1}{ptmcm}{b}{n}
% \SetSymbolFont{letters}{bold}{OML}{ptmcm}{b}{it}
% \SetMathAlphabet{\mathbf}{bold}{\encodingdefault}{\rmdefault}{m}{n}%
% \SetMathAlphabet{\mathsf}{bold}{\encodingdefault}{\sfdefault}{b}{n}%
% \SetMathAlphabet{\mathrm}{bold}{\encodingdefault}{\rmdefault}{b}{n}%

%\thinmuskip=2.5mu
%\medmuskip=3.5mu plus 1mu minus 1mu
%\thickmuskip=4.5mu plus 1.5mu minus 1mu
%\DeclareSymbolFont{symbols}     {OMS}{cmsy}{m}{n}
%\DeclareSymbolFont{largesymbols}{OMX}{cmex}{m}{n}
%\SetSymbolFont{symbols}{bold}{OMS}{cmsy}{b}{n}
%\SetSymbolFont{largesymbols}{bold}{OMX}{cmex}{m}{n}

